A Large-Scale Benchmark and Risk Assessment of Traffic Analysis Attacks on Cloud LLM Services

Cloud-based Large language model (LLM) services create a network-level traffic side channel that can expose model, prompt, and task behavior despite encryption. From packet sizes, directions, timing, and burst structure alone, a passive local observer can infer the serving model, the user's prompt category, and the task executed by a collaborative multi-agent system. Yet current evidence is fragmented across separate datasets and settings, limiting reproducibility and comparison. We present, to our knowledge, the first unified measurement study and public benchmark of encrypted LLM traffic across both user--LLM and multi-agent executions. The large-scale benchmark contains 60,000 user--LLM interactions across 10 models and 6 prompt categories, plus 2,838 multi-agent executions covering 10 task categories and two coordination topologies. Using only encrypted packet metadata, we assess the risk of traffic analysis attack by characterizing traffic signatures, identifying the features most associated with leakage, and testing robustness under prompt reformulation, decoding-temperature changes, larger candidate model sets, and partial traffic observation. Model fingerprinting achieves 97.7\% balanced accuracy, prompt-category fingerprinting reaches 76.7\% mean accuracy, and multi-agent task fingerprinting achieves up to 90.7\% accuracy. Prompt reformulation weakens but does not remove model-specific leakage, and task fingerprints remain detectable even from a single agent's traffic.

==> sections/other_evalautions.tex <==

\subsection{Feature-Importance Analysis}
\label{sec:feature-importance}


\begin{table}[t]
\centering
\caption{Features used for user--LLM model fingerprinting, ordered by
their mean permutation importance across prompt categories.}
\label{tab:user-llm-features}
\small
\begin{tabular}{c p{0.8\columnwidth}}
\toprule
\textbf{No.} & \textbf{Feature description} \\
\midrule
1  & 25th percentile of response packet inter-arrival times. \\
2  & Median response packet inter-arrival time. \\
3  & Maximum response packet inter-arrival time. \\
4  & Mean response packet size. \\
5  & 75th percentile of response packet inter-arrival times. \\
6  & Standard deviation of response packet sizes. \\
7  & Median response packet size. \\
8  & Duration of the LLM response. \\
9  & Median response-burst duration. \\
10 & 75th percentile of response packet sizes. \\
11 & Number of response packets per second. \\
12 & Mean response packet inter-arrival time. \\
13 & Standard deviation of response packet inter-arrival times. \\
14 & Time from the final request packet to the first response packet. \\
15 & Number of response bytes per second. \\
16 & Total response payload bytes. \\
17 & Maximum response packet size. \\
18 & Number of response bursts. \\
19 & Number of response packets. \\
20 & Median number of bytes per response burst. \\
\bottomrule
\end{tabular}
\end{table}



We use permutation importance to identify which observable traffic
characteristics contribute most strongly to fingerprinting. Unlike the
Random-Forest impurity score, permutation importance is model-agnostic and
measures the effect of a feature directly on held-out classification
performance. For each test fold, we first calculate the balanced accuracy of
the trained classifier. We then randomly permute one feature while leaving all
other features unchanged and measure the resulting decrease in balanced
accuracy. A large decrease indicates that the classifier relies strongly on
that feature. We repeat the permutation multiple times to capture variability
and rank the features by their mean importance. Negative values indicate that
permuting a feature occasionally improves test performance and therefore
provide no evidence that the feature contributes reliably to fingerprinting.


Figure~\ref{fig:user-llm-feature-importance} shows that response timing is the
strongest source of information for distinguishing LLMs. In particular, the
lower quantile, median, and maximum of response-packet inter-arrival times
occupy the highest ranks. Response packet-size statistics and response
duration provide additional information, whereas aggregate volume features,
such as the total number of response packets and bytes, have substantially
smaller importance. These results suggest that LLM identity is exposed mainly
through differences in response-generation and streaming behavior rather than
traffic volume alone.




\begin{table}[t]
\centering
\caption{Multi-agent traffic features ranked by their mean permutation
importance on the MARBLE dataset.}
\label{tab:multi-agent-features}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{\columnwidth}{@{}c X@{}}
\toprule
\textbf{Rank} & \textbf{Feature description} \\
\midrule
1  & Median duration of directional traffic bursts. \\
2  & Maximum number of packets observed within a one-second interval. \\
3  & Incoming bytes as a fraction of all transmitted bytes. \\
4  & Fraction of execution time spent in idle gaps. \\
5  & Number of changes in packet direction. \\
6  & Median number of bytes per directional burst. \\
7  & Incoming packets as a fraction of all packets. \\
8  & Median packet inter-arrival time. \\
9  & Total number of directional traffic bursts. \\
10 & Average number of transmitted bytes per second. \\
11 & Total number of packets in the multi-agent execution. \\
12 & Median number of packets per burst. \\
13 & Standard deviation of packet inter-arrival times. \\
14 & 75th percentile of packet inter-arrival times. \\
15 & Number of activity episodes separated by idle gaps. \\
16 & Complete task-execution duration. \\
17 & Total number of transmitted bytes. \\
18 & Average number of packets per second. \\
19 & Mean packet count across one-second intervals. \\
20 & Median delay between consecutive bursts. \\
\bottomrule
\end{tabularx}
\end{table}



As shown in Figure~\ref{fig:multi-agent-feature-importance}, multi-agent task
fingerprinting relies most strongly on burst duration, peak packet activity,
the fraction of incoming bytes, and idle-time behavior. These characteristics
capture the interaction structure and activity pattern of a multi-agent
execution. The wide distributions reflect the limited size of the MARBLE
dataset and variation across evaluation folds. Features with importance near
or below zero do not provide a stable independent contribution under the
current evaluation and should not be interpreted as negatively associated
with a task.






\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]
    {img/user_llm_numbered_importance.pdf}
    \caption{Permutation importance for LLM-model fingerprinting in the
    user--LLM setting. The results are aggregated across the six prompt
    categories. Each feature number corresponds to its rank in
    Table~\ref{tab:user-llm-features}, with rank~1 denoting the largest mean
    decrease in balanced accuracy. The boxes summarize the variation across
    grouped cross-validation folds and repeated permutations.}
    \label{fig:user-llm-feature-importance}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]
    {img/multi_agent_numbered_importance.pdf}
    \caption{Permutation importance for multi-agent task fingerprinting on
    the 53 real MARBLE captures. Each feature number corresponds to its rank
    in Table~\ref{tab:multi-agent-features}. Importance is measured as the
    decrease in held-out balanced accuracy after permuting the feature.}
    \label{fig:multi-agent-feature-importance}
\end{figure}


